Data-Driven Probabilistic Energy Consumption Estimation for Battery Electric Vehicles with Model Uncertainty

This paper presents a novel probabilistic data-driven approach to trip-level energy consumption estimation of battery electric vehicles (BEVs). As there are very few electric vehicle (EV) charging stations, EV trip energy consumption estimation can make EV routing and charging planning easier for drivers. In this research article, we propose a new driver behaviour-centric EV energy consumption estimation model using probabilistic neural networks with model uncertainty. By incorporating model uncertainty into neural networks, we have created an ensemble of neural networks using Monte Carlo approximation. Our method comprehensively considers various vehicle dynamics, driver behaviour and environmental factors to estimate EV energy consumption for a given trip. We propose relative positive acceleration (RPA), average acceleration and average deceleration as driver behaviour factors in EV energy consumption estimation and this paper shows that the use of these driver behaviour features improves the accuracy of the EV energy consumption model significantly. Instead of predicting a single-point estimate for EV trip energy consumption, this proposed method predicts a probability distribution for the EV trip energy consumption. The experimental results of our approach show that our proposed probabilistic neural network with weight uncertainty achieves a mean absolute percentage error of 9.3% and outperforms other existing EV energy consumption models in terms of accuracy.

==> Data/VDM1.tex <==
c1,c2,c3
20.000000,1.000000,0.177121
20.000000,2.000000,0.178680
20.000000,3.000000,0.180240
20.000000,4.000000,0.181800
20.000000,5.000000,0.182436
20.000000,6.000000,0.182983
20.000000,7.000000,0.183529
20.000000,8.000000,0.184076
20.000000,9.000000,0.184622
20.000000,10.000000,0.185169
20.000000,11.000000,0.185715
20.000000,12.000000,0.186262
20.000000,13.000000,0.186808
20.000000,14.000000,0.187355
20.000000,15.000000,0.187901
20.000000,16.000000,0.188448
20.000000,17.000000,0.188994
20.000000,18.000000,0.189541
20.000000,19.000000,0.190088
20.000000,20.000000,0.190634
20.000000,21.000000,0.191181
20.000000,22.000000,0.191727
20.000000,23.000000,0.192274
20.000000,24.000000,0.192820
20.000000,25.000000,0.193367
20.000000,26.000000,0.194277
20.000000,27.000000,0.195434
20.000000,28.000000,0.196590
20.000000,29.000000,0.197746
21.000000,1.000000,0.178204
21.000000,2.000000,0.179763
21.000000,3.000000,0.181323
21.000000,4.000000,0.182497
21.000000,5.000000,0.183044
21.000000,6.000000,0.183590
21.000000,7.000000,0.184137
21.000000,8.000000,0.184684
21.000000,9.000000,0.185230
21.000000,10.000000,0.185777
21.000000,11.000000,0.186323
21.000000,12.000000,0.186870
21.000000,13.000000,0.187416
21.000000,14.000000,0.187963
21.000000,15.000000,0.188509
21.000000,16.000000,0.189056
21.000000,17.000000,0.189602
21.000000,18.000000,0.190149
21.000000,19.000000,0.190695
21.000000,20.000000,0.191242
21.000000,21.000000,0.191788
21.000000,22.000000,0.192335
21.000000,23.000000,0.192882
21.000000,24.000000,0.193428
21.000000,25.000000,0.194064
21.000000,26.000000,0.195220
21.000000,27.000000,0.196376
21.000000,28.000000,0.197533
21.000000,29.000000,0.198689
22.000000,1.000000,0.179287
22.000000,2.000000,0.180846
22.000000,3.000000,0.182406
22.000000,4.000000,0.183105
22.000000,5.000000,0.183652
22.000000,6.000000,0.184198
22.000000,7.000000,0.184745
22.000000,8.000000,0.185291
22.000000,9.000000,0.185838
22.000000,10.000000,0.186384
22.000000,11.000000,0.186931
22.000000,12.000000,0.187477
22.000000,13.000000,0.188024
22.000000,14.000000,0.188571
22.000000,15.000000,0.189117
22.000000,16.000000,0.189664
22.000000,17.000000,0.190210
22.000000,18.000000,0.190757
22.000000,19.000000,0.191303
22.000000,20.000000,0.191850
22.000000,21.000000,0.192396
22.000000,22.000000,0.192943
22.000000,23.000000,0.193489
22.000000,24.000000,0.194036
22.000000,25.000000,0.195006
22.000000,26.000000,0.196163
22.000000,27.000000,0.197319
22.000000,28.000000,0.198476
22.000000,29.000000,0.199632
23.000000,1.000000,0.180370
23.000000,2.000000,0.181929
23.000000,3.000000,0.183166
23.000000,4.000000,0.183713
23.000000,5.000000,0.184260
23.000000,6.000000,0.184806
23.000000,7.000000,0.185353
23.000000,8.000000,0.185899
23.000000,9.000000,0.186446
23.000000,10.000000,0.186992
23.000000,11.000000,0.187539
23.000000,12.000000,0.188085
23.000000,13.000000,0.188632
23.000000,14.000000,0.189178
23.000000,15.000000,0.189725
23.000000,16.000000,0.190272
23.000000,17.000000,0.190818
23.000000,18.000000,0.191365
23.000000,19.000000,0.191911
23.000000,20.000000,0.192458
23.000000,21.000000,0.193004
23.000000,22.000000,0.193551
23.000000,23.000000,0.194097
23.000000,24.000000,0.194793
23.000000,25.000000,0.195949
23.000000,26.000000,0.197106
23.000000,27.000000,0.198262
23.000000,28.000000,0.199418
23.000000,29.000000,0.200575
24.000000,1.000000,0.181453
24.000000,2.000000,0.183012
24.000000,3.000000,0.183774
24.000000,4.000000,0.184321
24.000000,5.000000,0.184867
24.000000,6.000000,0.185414
24.000000,7.000000,0.185960
24.000000,8.000000,0.186507
24.000000,9.000000,0.187054
24.000000,10.000000,0.187600
24.000000,11.000000,0.188147
24.000000,12.000000,0.188693
24.000000,13.000000,0.189240
24.000000,14.000000,0.189786
24.000000,15.000000,0.190333
24.000000,16.000000,0.190879
24.000000,17.000000,0.191426
24.000000,18.000000,0.191972
24.000000,19.000000,0.192519
24.000000,20.000000,0.193065
24.000000,21.000000,0.193612
24.000000,22.000000,0.194159
24.000000,23.000000,0.194705
24.000000,24.000000,0.195735
24.000000,25.000000,0.196892
24.000000,26.000000,0.198048
24.000000,27.000000,0.199205
24.000000,28.000000,0.200361
24.000000,29.000000,0.201517
25.000000,1.000000,0.182536
25.000000,2.000000,0.183836
25.000000,3.000000,0.184382
25.000000,4.000000,0.184929
25.000000,5.000000,0.185475
25.000000,6.000000,0.186022
25.000000,7.000000,0.186568
25.000000,8.000000,0.187115
25.000000,9.000000,0.187661
25.000000,10.000000,0.188208
25.000000,11.000000,0.188754
25.000000,12.000000,0.189301
25.000000,13.000000,0.189848
25.000000,14.000000,0.190394
25.000000,15.000000,0.190941
25.000000,16.000000,0.191487
25.000000,17.000000,0.192034
25.000000,18.000000,0.192580
25.000000,19.000000,0.193127
25.000000,20.000000,0.193673
25.000000,21.000000,0.194220
25.000000,22.000000,0.194766
25.000000,23.000000,0.195522
25.000000,24.000000,0.196678
25.000000,25.000000,0.197835
25.000000,26.000000,0.198991
25.000000,27.000000,0.200147
25.000000,28.000000,0.201304
25.000000,29.000000,0.202460
26.000000,1.000000,0.183618
26.000000,2.000000,0.184443
26.000000,3.000000,0.184990
26.000000,4.000000,0.185536
26.000000,5.000000,0.186083
26.000000,6.000000,0.186630
26.000000,7.000000,0.187176
26.000000,8.000000,0.187723
26.000000,9.000000,0.188269
26.000000,10.000000,0.188816
26.000000,11.000000,0.189362
26.000000,12.000000,0.189909
26.000000,13.000000,0.190455
26.000000,14.000000,0.191002
26.000000,15.000000,0.191548
26.000000,16.000000,0.192095
26.000000,17.000000,0.192641
26.000000,18.000000,0.193188
26.000000,19.000000,0.193735
26.000000,20.000000,0.194281
26.000000,21.000000,0.194828
26.000000,22.000000,0.195374
26.000000,23.000000,0.196465
26.000000,24.000000,0.197621
26.000000,25.000000,0.198777
26.000000,26.000000,0.199934
26.000000,27.000000,0.201090
26.000000,28.000000,0.202247
26.000000,29.000000,0.203403
27.000000,1.000000,0.184505
27.000000,2.000000,0.185051
27.000000,3.000000,0.185598
27.000000,4.000000,0.186144
27.000000,5.000000,0.186691
27.000000,6.000000,0.187237
27.000000,7.000000,0.187784
27.000000,8.000000,0.188330
27.000000,9.000000,0.188877
27.000000,10.000000,0.189424
27.000000,11.000000,0.189970
27.000000,12.000000,0.190517
27.000000,13.000000,0.191063
27.000000,14.000000,0.191610
27.000000,15.000000,0.192156
27.000000,16.000000,0.192703
27.000000,17.000000,0.193249
27.000000,18.000000,0.193796
27.000000,19.000000,0.194342
27.000000,20.000000,0.194889
27.000000,21.000000,0.195435
27.000000,22.000000,0.196251
27.000000,23.000000,0.197407
27.000000,24.000000,0.198564
27.000000,25.000000,0.199720
27.000000,26.000000,0.200876
27.000000,27.000000,0.202033
27.000000,28.000000,0.203189
27.000000,29.000000,0.204346
28.000000,1.000000,0.185113
28.000000,2.000000,0.185659
28.000000,3.000000,0.186206
28.000000,4.000000,0.186752
28.000000,5.000000,0.187299
28.000000,6.000000,0.187845
28.000000,7.000000,0.188392
28.000000,8.000000,0.188938
28.000000,9.000000,0.189485
28.000000,10.000000,0.190031
28.000000,11.000000,0.190578
28.000000,12.000000,0.191124
28.000000,13.000000,0.191671
28.000000,14.000000,0.192218
28.000000,15.000000,0.192764
28.000000,16.000000,0.193311
28.000000,17.000000,0.193857
28.000000,18.000000,0.194404
28.000000,19.000000,0.194950
28.000000,20.000000,0.195497
28.000000,21.000000,0.196043
28.000000,22.000000,0.197194
28.000000,23.000000,0.198350
28.000000,24.000000,0.199506
28.000000,25.000000,0.200663
28.000000,26.000000,0.201819
28.000000,27.000000,0.202976
28.000000,28.000000,0.204132
28.000000,29.000000,0.205288
29.000000,1.000000,0.185720
29.000000,2.000000,0.186267
29.000000,3.000000,0.186813
29.000000,4.000000,0.187360
29.000000,5.000000,0.187906
29.000000,6.000000,0.188453
29.000000,7.000000,0.189000
29.000000,8.000000,0.189546
29.000000,9.000000,0.190093
29.000000,10.000000,0.190639
29.000000,11.000000,0.191186
29.000000,12.000000,0.191732
29.000000,13.000000,0.192279
29.000000,14.000000,0.192825
29.000000,15.000000,0.193372
29.000000,16.000000,0.193918
29.000000,17.000000,0.194465
29.000000,18.000000,0.195011
29.000000,19.000000,0.195558
29.000000,20.000000,0.196105
29.000000,21.000000,0.196980
29.000000,22.000000,0.198136
29.000000,23.000000,0.199293
29.000000,24.000000,0.200449
29.000000,25.000000,0.201606
29.000000,26.000000,0.202762
29.000000,27.000000,0.203918
29.000000,28.000000,0.205075
29.000000,29.000000,0.206231
30.000000,1.000000,0.186328
30.000000,2.000000,0.186875
30.000000,3.000000,0.187421
30.000000,4.000000,0.187968
30.000000,5.000000,0.188514
30.000000,6.000000,0.189061
30.000000,7.000000,0.189607
30.000000,8.000000,0.190154
30.000000,9.000000,0.190700
30.000000,10.000000,0.191247
30.000000,11.000000,0.191794
30.000000,12.000000,0.192340
30.000000,13.000000,0.192887
30.000000,14.000000,0.193433
30.000000,15.000000,0.193980
30.000000,16.000000,0.194526
30.000000,17.000000,0.195073
30.000000,18.000000,0.195619
30.000000,19.000000,0.196166
30.000000,20.000000,0.196766
30.000000,21.000000,0.197923
30.000000,22.000000,0.199079
30.000000,23.000000,0.200236
30.000000,24.000000,0.201392
30.000000,25.000000,0.202548
30.000000,26.000000,0.203705
30.000000,27.000000,0.204861
30.000000,28.000000,0.206017
30.000000,29.000000,0.207174
31.000000,1.000000,0.186936
31.000000,2.000000,0.187483
31.000000,3.000000,0.188029
31.000000,4.000000,0.188576
31.000000,5.000000,0.189122
31.000000,6.000000,0.189669
31.000000,7.000000,0.190215
31.000000,8.000000,0.190762
31.000000,9.000000,0.191308
31.000000,10.000000,0.191855
31.000000,11.000000,0.192401
31.000000,12.000000,0.192948
31.000000,13.000000,0.193494
31.000000,14.000000,0.194041
31.000000,15.000000,0.194588
31.000000,16.000000,0.195134
31.000000,17.000000,0.195681
31.000000,18.000000,0.196227
31.000000,19.000000,0.196774
31.000000,20.000000,0.197709
31.000000,21.000000,0.198866
31.000000,22.000000,0.200022
31.000000,23.000000,0.201178
31.000000,24.000000,0.202335
31.000000,25.000000,0.203491
31.000000,26.000000,0.204647
31.000000,27.000000,0.205804
31.000000,28.000000,0.206960
31.000000,29.000000,0.208117
32.000000,1.000000,0.187544
32.000000,2.000000,0.188090
32.000000,3.000000,0.188637
32.000000,4.000000,0.189183
32.000000,5.000000,0.189730
32.000000,6.000000,0.190277
32.000000,7.000000,0.190823
32.000000,8.000000,0.191370
32.000000,9.000000,0.191916
32.000000,10.000000,0.192463
32.000000,11.000000,0.193009
32.000000,12.000000,0.193556
32.000000,13.000000,0.194102
32.000000,14.000000,0.194649
32.000000,15.000000,0.195195
32.000000,16.000000,0.195742
32.000000,17.000000,0.196288
32.000000,18.000000,0.196835
32.000000,19.000000,0.197496
32.000000,20.000000,0.198652
32.000000,21.000000,0.199808
32.000000,22.000000,0.200965
32.000000,23.000000,0.202121
32.000000,24.000000,0.203277
32.000000,25.000000,0.204434
32.000000,26.000000,0.205590
32.000000,27.000000,0.206747
32.000000,28.000000,0.207903
32.000000,29.000000,0.209059
33.000000,1.000000,0.188152
33.000000,2.000000,0.188698
33.000000,3.000000,0.189245
33.000000,4.000000,0.189791
33.000000,5.000000,0.190338
33.000000,6.000000,0.190884
33.000000,7.000000,0.191431
33.000000,8.000000,0.191977
33.000000,9.000000,0.192524
33.000000,10.000000,0.193071
33.000000,11.000000,0.193617
33.000000,12.000000,0.194164
33.000000,13.000000,0.194710
33.000000,14.000000,0.195257
33.000000,15.000000,0.195803
33.000000,16.000000,0.196350
33.000000,17.000000,0.196896
33.000000,18.000000,0.197443
33.000000,19.000000,0.198438
33.000000,20.000000,0.199595
33.000000,21.000000,0.200751
33.000000,22.000000,0.201907
33.000000,23.000000,0.203064
33.000000,24.000000,0.204220
33.000000,25.000000,0.205377
33.000000,26.000000,0.206533
33.000000,27.000000,0.207689
33.000000,28.000000,0.208846
33.000000,29.000000,0.210002
34.000000,1.000000,0.188759
34.000000,2.000000,0.189306
34.000000,3.000000,0.189853
34.000000,4.000000,0.190399
34.000000,5.000000,0.190946
34.000000,6.000000,0.191492
34.000000,7.000000,0.192039
34.000000,8.000000,0.192585
34.000000,9.000000,0.193132
34.000000,10.000000,0.193678
34.000000,11.000000,0.194225
34.000000,12.000000,0.194771
34.000000,13.000000,0.195318
34.000000,14.000000,0.195865
34.000000,15.000000,0.196411
34.000000,16.000000,0.196958
34.000000,17.000000,0.197504
34.000000,18.000000,0.198225
34.000000,19.000000,0.199381
34.000000,20.000000,0.200537
34.000000,21.000000,0.201694
34.000000,22.000000,0.202850
34.000000,23.000000,0.204006
34.000000,24.000000,0.205163
34.000000,25.000000,0.206319
34.000000,26.000000,0.207476
34.000000,27.000000,0.208632
34.000000,28.000000,0.209788
34.000000,29.000000,0.210945
35.000000,1.000000,0.189367
35.000000,2.000000,0.189914
35.000000,3.000000,0.190460
35.000000,4.000000,0.191007
35.000000,5.000000,0.191553
35.000000,6.000000,0.192100
35.000000,7.000000,0.192647
35.000000,8.000000,0.193193
35.000000,9.000000,0.193740
35.000000,10.000000,0.194286
35.000000,11.000000,0.194833
35.000000,12.000000,0.195379
35.000000,13.000000,0.195926
35.000000,14.000000,0.196472
35.000000,15.000000,0.197019
35.000000,16.000000,0.197565
35.000000,17.000000,0.198112
35.000000,18.000000,0.199167
35.000000,19.000000,0.200324
35.000000,20.000000,0.201480
35.000000,21.000000,0.202636
35.000000,22.000000,0.203793
35.000000,23.000000,0.204949
35.000000,24.000000,0.206106
35.000000,25.000000,0.207262
35.000000,26.000000,0.208418
35.000000,27.000000,0.209575
35.000000,28.000000,0.210731
35.000000,29.000000,0.211887
36.000000,1.000000,0.189975
36.000000,2.000000,0.190522
36.000000,3.000000,0.191068
36.000000,4.000000,0.191615
36.000000,5.000000,0.192161
36.000000,6.000000,0.192708
36.000000,7.000000,0.193254
36.000000,8.000000,0.193801
36.000000,9.000000,0.194347
36.000000,10.000000,0.194894
36.000000,11.000000,0.195441
36.000000,12.000000,0.195987
36.000000,13.000000,0.196534
36.000000,14.000000,0.197080
36.000000,15.000000,0.197627
36.000000,16.000000,0.198173
36.000000,17.000000,0.198954
36.000000,18.000000,0.200110
36.000000,19.000000,0.201266
36.000000,20.000000,0.202423
36.000000,21.000000,0.203579
36.000000,22.000000,0.204736
36.000000,23.000000,0.205892
36.000000,24.000000,0.207048
36.000000,25.000000,0.208205
36.000000,26.000000,0.209361
36.000000,27.000000,0.210517
36.000000,28.000000,0.211674
36.000000,29.000000,0.212830
37.000000,1.000000,0.190583
37.000000,2.000000,0.191130
37.000000,3.000000,0.191676
37.000000,4.000000,0.192223
37.000000,5.000000,0.192769
37.000000,6.000000,0.193316
37.000000,7.000000,0.193862
37.000000,8.000000,0.194409
37.000000,9.000000,0.194955
37.000000,10.000000,0.195502
37.000000,11.000000,0.196048
37.000000,12.000000,0.196595
37.000000,13.000000,0.197141
37.000000,14.000000,0.197688
37.000000,15.000000,0.198234
37.000000,16.000000,0.198781
37.000000,17.000000,0.199896
37.000000,18.000000,0.201053
37.000000,19.000000,0.202209
37.000000,20.000000,0.203366
37.000000,21.000000,0.204522
37.000000,22.000000,0.205678
37.000000,23.000000,0.206835
37.000000,24.000000,0.207991
37.000000,25.000000,0.209147
37.000000,26.000000,0.210304
37.000000,27.000000,0.211460
37.000000,28.000000,0.212617
37.000000,29.000000,0.214021
38.000000,1.000000,0.191191
38.000000,2.000000,0.191737
38.000000,3.000000,0.192284
38.000000,4.000000,0.192830
38.000000,5.000000,0.193377
38.000000,6.000000,0.193923
38.000000,7.000000,0.194470
38.000000,8.000000,0.195017
38.000000,9.000000,0.195563
38.000000,10.000000,0.196110
38.000000,11.000000,0.196656
38.000000,12.000000,0.197203
38.000000,13.000000,0.197749
38.000000,14.000000,0.198296
38.000000,15.000000,0.198842
38.000000,16.000000,0.199683
38.000000,17.000000,0.200839
38.000000,18.000000,0.201996
38.000000,19.000000,0.203152
38.000000,20.000000,0.204308
38.000000,21.000000,0.205465
38.000000,22.000000,0.206621
38.000000,23.000000,0.207777
38.000000,24.000000,0.208934
38.000000,25.000000,0.210090
38.000000,26.000000,0.211247
38.000000,27.000000,0.212403
38.000000,28.000000,0.213559
38.000000,29.000000,0.216091
39.000000,1.000000,0.191799
39.000000,2.000000,0.192345
39.000000,3.000000,0.192892
39.000000,4.000000,0.193438
39.000000,5.000000,0.193985
39.000000,6.000000,0.194531
39.000000,7.000000,0.195078
39.000000,8.000000,0.195624
39.000000,9.000000,0.196171
39.000000,10.000000,0.196717
39.000000,11.000000,0.197264
39.000000,12.000000,0.197811
39.000000,13.000000,0.198357
39.000000,14.000000,0.198904
39.000000,15.000000,0.199469
39.000000,16.000000,0.200626
39.000000,17.000000,0.201782
39.000000,18.000000,0.202938
39.000000,19.000000,0.204095
39.000000,20.000000,0.205251
39.000000,21.000000,0.206407
39.000000,22.000000,0.207564
39.000000,23.000000,0.208720
39.000000,24.000000,0.209877
39.000000,25.000000,0.211033
39.000000,26.000000,0.212189
39.000000,27.000000,0.213346
39.000000,28.000000,0.214502
39.000000,29.000000,0.218161

